Tracking Objects Through Assembly and Decomposition

Tracking objects through transformations is essential for understanding real-world dynamics. Recent work has extended traditional object tracking to detect state changes. However, existing methods require an initial object prompt and detect only its decompositions, missing assembly events, which begin with multiple objects rather than one. We therefore introduce a prompt-free formulation of this task, where the goal is to recover all object tracks and detect both decomposition and assembly events given only a video. Our key insight is that assembly is decomposition in reverse. Building on this insight, we present Atlas, a zero-shot system that constructs and jointly reasons over forward and reverse spatiotemporal partitions to recover object tracks and their transformations. We further introduce OmniST, a benchmark with dense annotations of objects and both transformation types. On OmniST, Atlas recovers more than twice as many state changes as prior methods while remaining competitive on existing benchmarks that only evaluate decomposition.

==> sections/06_acknowledgement.tex <==
\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2026/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}
